Structure of cosmic web in non-linear regime: the nearest neighbour and spherical contact distributions

In non-linear scales, the matter density distribution is not Gaussian. Consequently, the widely used two-point correlation function is not adequate anymore to capture the matter density field's entire behaviour. Among all statistics beyond correlation functions, the spherical contact (or equivalently void function), and nearest neighbour distribution function seem promising tools to probe matter distribution in non-linear regime. In this work, we use halos from cosmological N-body simulations, galaxy groups from the volume-limited galaxy group and central galaxies from mock galaxy catalogues, to compare the spherical contact with the nearest neighbour distribution functions. We also calculate the J-function (or equivalently the first conditional correlation function), for different samples. Moreover, we consider the redshift evolution and mass-scale dependence of statistics in the simulations and dependence on the magnitude of volume-limited samples in group catalogues as well as the mock central galaxies. The shape of the spherical contact probability distribution function is nearly skew-normal, with skewness and kurtosis being approximately 0.5 and 3, respectively. On the other hand, the nearest neighbour probability distribution function is nearly log-normal, with logarithmic skewness and kurtosis being approximately 0.1 and 2.5, respectively. Accordingly, the spherical contact distribution function probes larger scales compared to the nearest neighbour distribution function, which is influenced by details of structures. We also find a linear relation between the mean and variance of the spherical contact probability distribution function in simulations and mock galaxies, which could be used as a distinguishing probe of cosmological models.

==> Bib.tex <==
@article{abbott2018dark,
  title={Dark Energy Survey year 1 results: Cosmological constraints from galaxy clustering and weak lensing},
  author={Abbott, TMC and Abdalla, Filipe B and Alarcon, A and Aleksi{\'c}, J and Allam, Sahar and Allen, Steven and Amara, A and Annis, James and Asorey, J and Avila, S and others},
  journal={Physical Review D},
  volume={98},
  number={4},
  pages={043526},
  year={2018},
  publisher={APS}
}

@article{Abbott:2017wau,
    author = "Abbott, T. M. C. and others",
    collaboration = "DES",
    title = "{Dark Energy Survey year 1 results: Cosmological constraints from galaxy clustering and weak lensing}",
    eprint = "1708.01530",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "FERMILAB-PUB-17-294-PPD",
    doi = "10.1103/PhysRevD.98.043526",
    journal = "Phys. Rev. D",
    volume = "98",
    number = "4",
    pages = "043526",
    year = "2018"
}

@article{ade2014planck,
  title={Planck 2013 results. XVI. Cosmological parameters},
  author={Ade, Peter AR and Aghanim, N and Armitage-Caplan, C and Arnaud, M and Ashdown, M and Atrio-Barandela, F and Aumont, J and Baccigalupi, C and Banday, Anthony J and Barreiro, RB and others},
  journal={Astronomy \& Astrophysics},
  volume={571},
  pages={A16},
  year={2014},
  publisher={EDP sciences}
}

@article{Ade:2013zuv,
    author = "Ade, P. A. R. and others",
    collaboration = "Planck",
    title = "{Planck 2013 results. XVI. Cosmological parameters}",
    eprint = "1303.5076",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "CERN-PH-TH-2013-129",
    doi = "10.1051/0004-6361/201321591",
    journal = "Astron. Astrophys.",
    volume = "571",
    pages = "A16",
    year = "2014"
}

@article{bond1996filaments,
  title={How filaments of galaxies are woven into the cosmic web},
  author={Bond, J Richard and Kofman, Lev and Pogosyan, Dmitry},
  journal={Nature},
  volume={380},
  number={6575},
  pages={603--606},
  year={1996},
  publisher={Nature Publishing Group}
}

@article{sefusatti2006cosmology,
  title={Cosmology and the bispectrum},
  author={Sefusatti, Emiliano and Crocce, Mart{\'\i}n and Pueblas, Sebasti{\'a}n and Scoccimarro, Rom{\'a}n},
  journal={Physical Review D},
  volume={74},
  number={2},
  pages={023522},
  year={2006},
  publisher={APS}
}

@article{verde2001trispectrum,
  title={On the trispectrum as a Gaussian test for cosmology},
  author={Verde, Licia and Heavens, Alan F},
  journal={The Astrophysical Journal},
  volume={553},
  number={1},
  pages={14},
  year={2001},
  publisher={IOP Publishing}
}

@article{Verde:2001pf,
    author = "Verde, Licia and Heavens, Alan F.",
    title = "{On the trispectrum as a Gaussian test for cosmology}",
    eprint = "astro-ph/0101143",
    archivePrefix = "arXiv",
    doi = "10.1086/320656",
    journal = "Astrophys. J.",
    volume = "553",
    pages = "14",
    year = "2001"
}

@article{scoccimarro1998nonlinear,
  title={Nonlinear evolution of the bispectrum of cosmological perturbations},
  author={Scoccimarro, Roman and Colombi, Stephane and Fry, James N and Frieman, Joshua A and Hivon, Eric and Melott, Adrian},
  journal={The Astrophysical Journal},
  volume={496},
  number={2},
  pages={586},
  year={1998},
  publisher={IOP Publishing}
}

@article{blake2014using,
  title={Using the topology of large-scale structure in the WiggleZ Dark Energy Survey as a cosmological standard ruler},
  author={Blake, Chris and James, J Berian and Poole, Gregory B},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={437},
  number={3},
  pages={2488--2506},
  year={2014},
  publisher={The Royal Astronomical Society}
}

@article{park2010large,
  title={Large-Scale Structure of the Universe as a Cosmic Standard Ruler},
  author={Park, Changbom and Kim, Young-Rae},
  journal={The Astrophysical Journal Letters},
  volume={715},
  number={2},
  pages={L185},
  year={2010},
  publisher={IOP Publishing}
}

@article{Riess_2019,
	doi = {10.3847/1538-4357/ab1422},
	url = {https://doi.org/10.3847/1538-4357/ab1422},
	year = 2019,
	month = {may},
	publisher = {American Astronomical Society},
	volume = {876},
	number = {1},
	pages = {85},
	author = {Adam G. Riess and Stefano Casertano and Wenlong Yuan and Lucas M. Macri and Dan Scolnic},
	title = {Large Magellanic Cloud Cepheid Standards Provide a 1{\%} Foundation for the Determination of the Hubble Constant and Stronger Evidence for Physics beyond $\{upLambda}${CDM}},
	journal = {The Astrophysical Journal},
	abstract = {We present an improved determination of the Hubble constant from Hubble Space Telescope (HST) observations of 70 long-period Cepheids in the Large Magellanic Cloud (LMC). These were obtained with the same WFC3 photometric system used to measure extragalactic Cepheids in the hosts of SNe Ia. Gyroscopic control of HST was employed to reduce overheads while collecting a large sample of widely separated Cepheids. The Cepheid period–luminosity relation provides a zero-point-independent link with 0.4% precision between the new 1.2% geometric distance to the LMC from detached eclipsing binaries (DEBs) measured by Pietrzyński et al. and the luminosity of SNe Ia. Measurements and analysis of the LMC Cepheids were completed prior to knowledge of the new DEB LMC distance. Combined with a refined calibration of the count-rate linearity of WFC3-IR with 0.1% precision, these three improved elements together reduce the overall uncertainty in the geometric calibration of the Cepheid distance ladder based on the LMC from 2.5% to 1.3%. Using only the LMC DEBs to calibrate the ladder, we find H
0 = 74.22 ± 1.82 km s−1 Mpc−1 including systematic uncertainties, 3% higher than before for this particular anchor. Combining the LMC DEBs, masers in NGC 4258, and Milky Way parallaxes yields our best estimate: H
0 = 74.03 ± 1.42 km s−1 Mpc−1, including systematics, an uncertainty of 1.91%–15% lower than our best previous result. Removing any one of these anchors changes H
0 by less than 0.7%. The difference between H
0 measured locally and the value inferred from Planck CMB and ΛCDM is 6.6 ± 1.5 km s−1 Mpc−1 or 4.4σ (P = 99.999% for Gaussian errors) in significance, raising the discrepancy beyond a plausible level of chance. We summarize independent tests showing that this discrepancy is not attributable to an error in any one source or measurement, increasing the odds that it results from a cosmological feature beyond ΛCDM.}
}

@article{10.1046/j.1365-8711.1998.01313.x,
    author = {Munshi, Dipak and Chiang, Lung-Yih and Coles, Peter and Melott, Adrian L.},
    title = "{Non-local scaling in two-dimensional gravitational clustering}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {293},
    number = {3},
    pages = {L68-L72},
    year = {1998},
    month = {01},
    abstract = "{Using an ensemble of high-resolution 2D numerical simulations, we explore the scaling properties of cosmological density fluctuations in the non-linear regime. We study the scaling behaviour of the usual N-point volume-averaged correlations, but also examine the scaling of the entire probability density function (PDF) of the fluctuations. We focus on two important issues: (i) whether the scaling behaviour of 2D clustering is consistent with what one infers from radial collapse arguments; and (ii) whether there is any evidence from these high-resolution simulations that a regime of stable clustering is ever entered. We find that the answers are (i) yes and (ii) no. We further find that the behaviour of the highly non-linear regime in these simulations suggests the existence of a regime in which the correlation function is independent of the initial power spectrum.}",
    issn = {0035-8711},
    doi = {10.1046/j.1365-8711.1998.01313.x},
    url = {https://doi.org/10.1046/j.1365-8711.1998.01313.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/293/3/L68/3882000/293-3-L68.pdf},
}

@article{Kerscher:1999gt,
    author = "Kerscher, Martin and Pons-Borderia, Maria Jesus and Schmalzing, Jens and Trasarti-Battistoni, Roberto and Buchert, Thomas and Martinez, Vicent J. and Valdarnini, Riccardo",
    title = "{A Global descriptor of spatial pattern interaction in the galaxy distribution}",
    eprint = "astro-ph/9712098",
    archivePrefix = "arXiv",
    doi = "10.1086/306902",
    journal = "Astrophys. J.",
    volume = "513",
    pages = "543--548",
    year = "1999"
}

@article{van1996nonparametric,
  title={A nonparametric measure of spatial interaction in point patterns},
  author={Van Lieshout, MNM and Baddeley, AJ},
  journal={Statistica Neerlandica},
  volume={50},
  number={3},
  pages={344--361},
  year={1996},
  publisher={Wiley Online Library}
}

@article{soneira1977there,
  title={Is there evidence for a spatially homogeneous population of field galaxies},
  author={Soneira, Raymond M and Peebles, PJE},
  journal={The Astrophysical Journal},
  volume={211},
  pages={1--15},
  year={1977}
}

@article{clark1954distance,
  title={Distance to nearest neighbor as a measure of spatial relationships in populations},
  author={Clark, Philip J and Evans, Francis C},
  journal={Ecology},
  volume={35},
  number={4},
  pages={445--453},
  year={1954},
  publisher={Wiley Online Library}
}

@book{martinez2001statistics,
  title={Statistics of the galaxy distribution},
  author={Martinez, Vicent J and Saar, Enn},
  year={2001},
  publisher={CRC press}
}

@book{chiu2013stochastic,
  title={Stochastic geometry and its applications},
  author={Chiu, Sung Nok and Stoyan, Dietrich and Kendall, Wilfrid S and Mecke, Joseph},
  year={2013},
  publisher={John Wiley \& Sons}
}

@book{baddeley2006stochastic,
  title={Stochastic Geometry: Lectures Given at the CIME Summer School Held in Martina Franca, Italy, September 13-18, 2004},
  author={Baddeley, Adrian and B{\'a}r{\'a}ny, Imre and Schneider, Rolf},
  year={2006},
  publisher={Springer}
}

@article{banerjee2021cosmological,
  title={Cosmological cross-correlations and nearest neighbor distributions},
  author={Banerjee, Arka and Abel, Tom},
  journal={arXiv preprint arXiv:2102.01184},
  year={2021}
}

@article{Banerjee:2021hkg,
    author = "Banerjee, Arka and Abel, Tom",
    title = "{Cosmological cross-correlations and nearest neighbor distributions}",
    eprint = "2102.01184",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "FERMILAB-PUB-21-029-T",
    month = "2",
    year = "2021"
}

@article{Banerjee:2020umh,
    author = "Banerjee, Arka and Abel, Tom",
    title = "{Nearest neighbour distributions: New statistical measures for cosmological clustering}",
    eprint = "2007.13342",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/staa3604",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "500",
    number = "4",
    pages = "5479--5499",
    year = "2020"
}

@article{Paranjape:2020wuc,
    author = "Paranjape, Aseem and Alam, Shadab",
    title = "{Voronoi volume function: A new probe of cosmology and galaxy evolution}",
    eprint = "2001.08760",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/staa1379",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "495",
    number = "3",
    pages = "3233--3251",
    year = "2020"
}

@article{Walsh:2019luq,
    author = "Walsh, Kilian and Tinker, Jeremy",
    title = "{Probing Galaxy Assembly Bias in BOSS Galaxies Using Void Probabilities}",
    eprint = "1905.07024",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stz1351",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "488",
    number = "1",
    pages = "470--479",
    year = "2019"
}

@article{10.1093/mnras/195.4.857,
    author = {Sharp, N. A.},
    title = "{‘Holes’ in the Zwicky catalogue}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {195},
    number = {4},
    pages = {857-867},
    year = {1981},
    month = {08},
    abstract = "{By applying an idea of White, we use the probability distributions of regions on the sky empty of galaxies, and of empty regions surrounding galaxies, to investigate the structure of the n-point correlation functions to quite high orders. The results are consistent with the suggestion \\$w\_n\\sim w\_2^\\{n-1\\}\\$.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/195.4.857},
    url = {https://doi.org/10.1093/mnras/195.4.857},
    eprint = {https://academic.oup.com/mnras/article-pdf/195/4/857/4861545/mnras195-0857.pdf},
}


@article{Fry:2013pma,
    author = "Fry, J. N. and Colombi, S.",
    title = "{Void Statistics and Hierarchical Scaling in the Halo Model}",
    eprint = "1305.5571",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stt745",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "433",
    pages = "581",
    year = "2013"
}

@article{Croton:2004ac,
    author = "Croton, D. J. and others",
    collaboration = "2dFGRS Team",
    title = "{The 2dF Galaxy Redshift Survey: Voids and hierarchical scaling models}",
    eprint = "astro-ph/0401406",
    archivePrefix = "arXiv",
    doi = "10.1111/j.1365-2966.2004.07968.x",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "352",
    pages = "828",
    year = "2004"
}

@ARTICLE{1991ApJ...369...30M,
       author = {{Maurogordato}, Sophie and {Lachieze-Rey}, Marc},
        title = "{Scaling Invariance in the Galaxy Distribution. II. Spatial and Luminosity Effects}",
      journal = {\apj},
     keywords = {Galactic Clusters, Galactic Evolution, Probability Density Functions, Astronomical Catalogs, Luminosity, Statistical Analysis, cosmology, galaxies: clustering, Astrophysics, COSMOLOGY, GALAXIES: CLUSTERING},
         year = 1991,
        month = mar,
       volume = {369},
        pages = {30},
          doi = {10.1086/169735},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1991ApJ...369...30M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{maurogordato1987void,
  title={Void probabilities in the galaxy distribution-Scaling and luminosity segregation},
  author={Maurogordato, Sophie and Lachieze-Rey, Marc},
  journal={The Astrophysical Journal},
  volume={320},
  pages={13--25},
  year={1987}
}

@ARTICLE{1986ApJ...306..358F,
       author = {{Fry}, J.~N.},
        title = "{Statistics of Voids in Hierarchical Universes}",
      journal = {\apj},
     keywords = {Cosmology, Galactic Clusters, Universe, Voids, Binomials, Computational Astrophysics, Hierarchies, Poisson Density Functions, Thermodynamics, Astrophysics, COSMOLOGY, GALAXIES: CLUSTERING},
         year = 1986,
        month = jul,
       volume = {306},
        pages = {358},
          doi = {10.1086/164348},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1986ApJ...306..358F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{munshi1999scaling,
  title={Scaling in gravitational clustering, two-and three-dimensional dynamics},
  author={Munshi, D and Bernardeau, F and Melott, AL and Schaeffer, R},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={303},
  number={3},
  pages={433--445},
  year={1999},
  publisher={Blackwell Science Ltd Oxford, UK}
}


@article{Jamieson:2020wxf,
    author = "Jamieson, Drew and Loverde, Marilena",
    title = "{Position-dependent matter density probability distribution function}",
    eprint = "2010.07235",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "YITP-SB-2020-33",
    doi = "10.1103/PhysRevD.102.123546",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "12",
    pages = "123546",
    year = "2020"
}


@article{Repp:2020kfd,
    author = "Repp, Andrew and Szapudi, Istv\'an",
    title = "{Galaxy Bias and $\sigma_8$ from Counts in Cells from the SDSS Main Sample}",
    eprint = "2006.01146",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnrasl/slaa139",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "498",
    number = "1",
    pages = "L125--L129",
    year = "2020"
}

@article{Friedrich:2019byw,
    author = "Friedrich, Oliver and Uhlemann, Cora and Villaescusa-Navarro, Francisco and Baldauf, Tobias and Manera, Marc and Nishimichi, Takahiro",
    title = "{Primordial non-Gaussianity without tails \textendash{} how to measure fNL with the bulk of the density PDF}",
    eprint = "1912.06621",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "YITP-19-122",
    doi = "10.1093/mnras/staa2160",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "498",
    number = "1",
    pages = "464--483",
    year = "2020"
}

@article{uhlemann2020fisher,
  title={Fisher for complements: extracting cosmology and neutrino mass from the counts-in-cells PDF},
  author={Uhlemann, Cora and Friedrich, Oliver and Villaescusa-Navarro, Francisco and Banerjee, Arka and Codis, Sandrine},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={495},
  number={4},
  pages={4006--4027},
  year={2020},
  publisher={Oxford University Press}
}


@article{10.1093/mnras/staa2073,
    author = {Mandal, Ankush and Nadkarni-Ghosh, Sharvari},
    title = "{One-point probability distribution function from spherical collapse: early dark energy versus ΛCDM}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {498},
    number = {1},
    pages = {355-372},
    year = {2020},
    month = {07},
    abstract = "{We compute the one-point probability distribution function (PDF) of an initially Gaussian dark matter density field using spherical collapse (SC). We compare the results to other forms available in the literature and also compare the PDFs in the Λ-cold dark matter model with an early dark energy (EDE) model. We find that the skewed lognormal distribution provides the best fit to the non-linear PDF from SC for both cosmologies, from a = 0.1 to 1 and for scales characterized by the comoving width of the Gaussian: σG = 0.5, 1, and 2. To elucidate the effect of cosmology, we examine the linear and non-linear growth rates through test cases. For overdensities, when the two models have the same initial density contrast, the differences due to cosmology are amplified in the non-linear regime, whereas, if the two models have the same linear density contrast today, then the differences in cosmology are damped in the non-linear regime. This behaviour is in contrast with voids, where the non-linear growth becomes ‘self-regulatory’ and is less sensitive to cosmology and initial conditions. To compare the PDFs, we examine the difference of the PDFs and evolution of the width of the PDF. The trends with scale and redshift are as expected. A tertiary aim of this paper was to check if the fitting form for the non-linear density–velocity divergence relation, derived for constant equation of state (w) models by Nadkarni-Ghosh holds for the EDE model. We find that it does with an accuracy of 4 per cent, thus increasing its range of validity.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/staa2073},
    url = {https://doi.org/10.1093/mnras/staa2073},
    eprint = {https://academic.oup.com/mnras/article-pdf/498/1/355/33710774/staa2073.pdf},
}

@article{Repp:2020etr,
    author = "Repp, Andrew and Szapudi, Istv\'an",
    title = "{The Variance and Covariance of Counts-in-Cells Probabilities}",
    eprint = "2007.00011",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/staa3237",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "500",
    number = "3",
    pages = "3631--3639",
    year = "2020"
}

@article{einasto2020evolution,
  title={Evolution of skewness and kurtosis of cosmic density fields},
  author={Einasto, Jaan and H{\"u}tsi, Gert and Liivam{\"a}gi, LJ and Einasto, Maret},
  journal={arXiv preprint arXiv:2011.13292},
  year={2020}
}

@article{Einasto:2020sqi,
    author = {Einasto, Jaan and H\"utsi, Gert and Liivam\"agi, L. J. and Einasto, Maret},
    title = "{Evolution of skewness and kurtosis of cosmic density fields}",
    eprint = "2011.13292",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    month = "11",
    year = "2020"
}



@article{Klypin:2017jjg,
    author = "Klypin, Anatoly and Prada, Francisco and Betancort-Rijo, Juan and Albareti, Franco D.",
    title = "{Density distribution of the cosmological matter field}",
    eprint = "1706.01909",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/sty2613",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "481",
    number = "4",
    pages = "4588--4601",
    year = "2018"
}

@article{shin2017new,
  title={New fitting formula for cosmic nonlinear density distribution},
  author={Shin, Jihye and Kim, Juhan and Pichon, Christophe and Jeong, Donghui and Park, Changbom},
  journal={The Astrophysical Journal},
  volume={843},
  number={1},
  pages={73},
  year={2017},
  publisher={IOP Publishing}
}

@article{gaztanaga2000gravitational,
  title={Gravitational evolution of the large-scale probability density distribution: the Edgeworth and Gamma expansions},
  author={Gaztanaga, E and Fosalba, P and Elizalde, E},
  journal={The Astrophysical Journal},
  volume={539},
  number={2},
  pages={522},
  year={2000},
  publisher={IOP Publishing}
}

@article{Colombi:1994sj,
    author = "Colombi, S.",
    title = "{A 'Skewed' lognormal approximation to the probability distribution function of the large scale density field}",
    eprint = "astro-ph/9402071",
    archivePrefix = "arXiv",
    reportNumber = "FERMILAB-PUB-94-050-A",
    doi = "10.1086/174834",
    journal = "Astrophys. J. Lett.",
    volume = "435",
    pages = "L536--539",
    year = "1994"
}


@article{10.1093/mnras/stw1074,
    author = {Uhlemann, C. and Codis, S. and Pichon, C. and Bernardeau, F. and Reimberg, P.},
    title = "{Back in the saddle: large-deviation statistics of the cosmic log-density field}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {460},
    number = {2},
    pages = {1529-1541},
    year = {2016},
    month = {05},
    abstract = "{We present a first principle approach to obtain analytical predictions for spherically averaged cosmic densities in the mildly non-linear regime that go well beyond what is usually achieved by standard perturbation theory. A large deviation principle allows us to compute the leading order cumulants of average densities in concentric cells. In this symmetry, the spherical collapse model leads to cumulant generating functions that are robust for finite variances and free of critical points when logarithmic density transformations are implemented. They yield in turn accurate density probability distribution functions (PDFs) from a straightforward saddle-point approximation valid for all density values. Based on this easy-to-implement modification, explicit analytic formulas for the evaluation of the one- and two-cell PDF are provided. The theoretical predictions obtained for the PDFs are accurate to a few per cent compared to the numerical integration, regardless of the density under consideration and in excellent agreement with N-body simulations for a wide range of densities. This formalism should prove valuable for accurately probing the quasi-linear scales of low-redshift surveys for arbitrary primordial power spectra.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stw1074},
    url = {https://doi.org/10.1093/mnras/stw1074},
    eprint = {https://academic.oup.com/mnras/article-pdf/460/2/1529/8116469/stw1074.pdf},
}


@article{10.1111/j.1365-2966.2008.13038.x,
    author = {Lam, Tsz Yan and Sheth, Ravi K.},
    title = "{Perturbation theory and excursion set estimates of the probability distribution function of dark matter, and a method for reconstructing the initial distribution function}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {386},
    number = {1},
    pages = {407-415},
    year = {2008},
    month = {03},
    abstract = "{Non-linear evolution is sometimes modelled by assuming there is a deterministic mapping from initial to final values of the locally smoothed overdensity. However, if an underdense region is embedded in a denser one, then it is possible that its evolution is determined by its surroundings, so the mapping between initial and final overdensities is not as ‘local’ as one might have assumed. If this source of non-locality is not accounted for, then it appears as stochasticity in the mapping between initial and final densities. Perturbation theory methods ignore this ‘cloud-in-cloud’ effect, whereas methods based on the excursion set approach do account for it; as a result, one may expect the two approaches to provide different estimates of the shape of the non-linear counts in cells distribution. We show that, on scales where the rms fluctuation is small, this source of non-locality has only a small effect, so the predictions of the two approaches differ only on the small scales on which perturbation theory is no longer expected to be valid anyway. We illustrate our results by comparing the predictions of these approaches when the initial–final mapping is given by the spherical collapse model. Both are in reasonably good agreement with measurements in numerical simulations on scales where the rms fluctuation is of the order of unity or smaller.If the deterministic mapping from initial conditions to final density depends on quantities other than the initial density, then this will also manifest as stochasticity in the mapping from initial density to final. For example, the Zeldovich approximation and the ellipsoidal collapse model both assume that the initial shear field plays an important role in determining the evolution. We compare the predictions of these approximations with simulations, both before and after accounting for the ‘cloud-in-cloud’ effect. Our analysis accounts approximately for the fact that the shape of a cell at the present time is different from its initial shape; ignoring this makes a noticeable difference on scales where the rms fluctuation in a cell is of the order of unity or larger.On scales where the rms fluctuation is 2 or less, methods based on the spherical model are sufficiently accurate to permit a rather accurate reconstruction of the shape of the initial distribution from the non-linear one. This can be used as the basis for a method for constraining the statistical properties of the initial fluctuation field from the present-day field, under the hypothesis that the evolution was purely gravitational. We illustrate by showing how the highly non-Gaussian non-linear density field in a numerical simulation can be transformed to provide an accurate estimate of the initial Gaussian distribution from which it evolved.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2008.13038.x},
    url = {https://doi.org/10.1111/j.1365-2966.2008.13038.x},
    eprint = {https://academic.oup.com/mnras/article-pdf/386/1/407/3012684/mnras0386-0407.pdf},
}


@article{Ivanov:2018lcg,
    author = "Ivanov, Mikhail M. and Kaurov, Alexander A. and Sibiryakov, Sergey",
    title = "{Non-perturbative probability distribution function for cosmological counts in cells}",
    eprint = "1811.07913",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "CERN-TH-2018-242, INR-TH-2018-027",
    doi = "10.1088/1475-7516/2019/03/009",
    journal = "JCAP",
    volume = "03",
    pages = "009",
    year = "2019"
}

@article{Bernardeau:2013dua,
    author = "Bernardeau, Francis and Pichon, Christophe and Codis, Sandrine",
    title = "{Statistics of cosmic density profiles from perturbation theory}",
    eprint = "1310.8134",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.90.103519",
    journal = "Phys. Rev. D",
    volume = "90",
    number = "10",
    pages = "103519",
    year = "2014"
}

@article{linde1982new,
  title={A new inflationary universe scenario: a possible solution of the horizon, flatness, homogeneity, isotropy and primordial monopole problems},
  author={Linde, Andrei D},
  journal={Physics Letters B},
  volume={108},
  number={6},
  pages={389--393},
  year={1982},
  publisher={Elsevier}
}

@article{guth1981inflationary,
  title={Inflationary universe: A possible solution to the horizon and flatness problems},
  author={Guth, Alan H},
  journal={Physical Review D},
  volume={23},
  number={2},
  pages={347},
  year={1981},
  publisher={APS}
}

@article{10.1093/mnras/280.3.754,
    author = {Ueda, Haruhiko and Yokoyama, Jun'ichi},
    title = "{Counts-in-cells analysis of the statistical distribution in an N-body simulated universe}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {280},
    number = {3},
    pages = {754-766},
    year = {1996},
    month = {06},
    abstract = "{Evolution of the statistical distribution of the density field is investigated by means of a counts-in-cells method in a low-density cold dark matter (CDM) simulated universe. Four model distributions, namely the negative binomial distribution, the lognormal distribution, the Edgeworth series and the skewed lognormal distribution, are tested to fit the calculated distribution function, and it is shown that only the skewed lognormal distribution of second- and third-order can describe the evolution of the statistical distribution perfectly well from the initially Gaussian regime to the present stage. The effect of sparse sampling is also investigated, and we conclude that in order to reconstruct the underlying density distribution we should use a sample with a galaxy number density larger than ∼ 0.01h−3 Mpc−3.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/280.3.754},
    url = {https://doi.org/10.1093/mnras/280.3.754},
    eprint = {https://academic.oup.com/mnras/article-pdf/280/3/754/3227708/280-3-754.pdf},
}

@article{10.1093/mnras/248.1.1,
    author = {Coles, Peter and Jones, Bernard},
    title = "{A lognormal model for the cosmological mass distribution}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {248},
    number = {1},
    pages = {1-13},
    year = {1991},
    month = {01},
    abstract = "{We discuss the use of a lognormal (LN) random field as a model for the distribution of matter in the Universe. We find a number of reasons why this should be a plausible approximation to the distribution of density irregularities obtained by evolving from Gaussian initial conditions. Unlike straightforward linear theory, the model always has \\$\\rho\\gt0\\$ but is arbitrarily close to the Gaussian at early times. It has the added advantage that, like the Gaussian model, all its statistical properties can be formulated in terms of one covariance function.A number of interesting and important difficulties with the statistical treatment of density perturbations are revealed by an analysis of this model. In particular, the LN model is not completely specified by its moments. We explain why this could be true for the actual matter field. We also show that the usual method of representing the three- and four-point correlation functions of galaxies, in terms of the parameters Q and R, is not useful for discriminating between Gaussian and non-Gaussian fluctuations, and propose better parameterizations in terms of the skewness and kurtosis of the three- and four-point distributions, respectively.Other characteristics of the model, such as topology (genus curves, etc.), multifractal behaviour, void probabilities and biasing (behaviour of ‘peaks’ relative to background fluctuations) are also discussed. The model also provides a way of checking the consistency of treatments of large-scale streaming motions in the Universe by allowing us to determine the scale at which linear theory cannot be accurate for both the matter and velocity fields.We discuss a possible model for the number-count distribution of galaxies, based on the LN distribution but allowing for discreteness effects which can make the distribution of log n appear non-Gaussian, and show how to construct Monte-Carlo simulations of point patterns (in one-, two, or three-dimensions) which contain correlations of all orders.}",
    issn = {0035-8711},
    doi = {10.1093/mnras/248.1.1},
    url = {https://doi.org/10.1093/mnras/248.1.1},
    eprint = {https://academic.oup.com/mnras/article-pdf/248/1/1/18194814/mnras248-0001.pdf},
}

@article{10.2307/40673267,
 ISSN = {00046280, 15383873},
 URL = {http://www.jstor.org/stable/40673267},
 author = {F. Zwicky},
 journal = {Publications of the Astronomical Society of the Pacific},
 number = {411},
 pages = {518--529},
 publisher = {[University of Chicago Press, Astronomical Society of the Pacific]},
 title = {NON-UNIFORMITIES IN THE APPARENT DISTRIBUTION OF CLUSTERS OF GALAXIES},
 volume = {69},
 year = {1957}
}


@BOOK{1936rene.book.....H,
       author = {{Hubble}, E.~P.},
        title = "{Realm of the Nebulae}",
         year = 1936,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1936rene.book.....H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{bernardeau1992gravity,
  title={The gravity-induced quasi-Gaussian correlation hierarchy},
  author={Bernardeau, Francis},
  journal={The Astrophysical Journal},
  volume={392},
  pages={1--14},
  year={1992}
}

@article{colley2015genus,
  title={Genus topology and cross-correlation of BICEP2 and Planck 353 GHz B-modes: further evidence favouring gravity wave detection},
  author={Colley, Wesley N and Gott III, J Richard},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={447},
  number={2},
  pages={2034--2045},
  year={2015},
  publisher={Oxford University Press}
}

@article{Colley:2014nna,
    author = "Colley, Wesley N. and Gott, J. Richard",
    title = "{Genus topology and cross-correlation of BICEP2 and Planck 353 GHz B-modes: further evidence favouring gravity wave detection}",
    eprint = "1409.4491",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stu2547",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "447",
    number = "2",
    pages = "2034--2045",
    year = "2015"
}

@article{appleby2018cosmological,
  title={Cosmological Parameter Estimation Using the Genus Amplitude?Application to Mock Galaxy Catalogs},
  author={Appleby, Stephen and Park, Changbom and Hong, Sungwook E and Kim, Juhan},
  journal={The Astrophysical Journal},
  volume={853},
  number={1},
  pages={17},
  year={2018},
  publisher={IOP Publishing}
}

@article{Appleby:2018jew,
    author = "Appleby, Stephen and Park, Changbom and Hong, Sungwook E. and Kim, Juhan",
    title = "{Cosmological Parameter Estimation Using the Genus Amplitude\textemdash{}Application to Mock Galaxy Catalogs}",
    eprint = "1801.06342",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.3847/1538-4357/aaa24f",
    journal = "Astrophys. J.",
    volume = "853",
    number = "1",
    pages = "17",
    year = "2018"
}

@article{gott1986sponge,
  title={The sponge-like topology of large-scale structure in the universe},
  author={Gott III, J Richard and Melott, Adrian L and Dickinson, Mark},
  journal={The Astrophysical Journal},
  volume={306},
  pages={341--357},
  year={1986}
}

@article{wang2012topology,
  title={Topology of a Large-scale Structure as a Test of Modified Gravity},
  author={Wang, Xin and Chen, Xuelei and Park, Changbom},
  journal={The Astrophysical Journal},
  volume={747},
  number={1},
  pages={48},
  year={2012},
  publisher={IOP Publishing}
}

@article{zunckel2011using,
  title={Using the topology of large-scale structure to constrain dark energy},
  author={Zunckel, Caroline and Gott III, J Richard and Lunnan, Ragnhild},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={412},
  number={2},
  pages={1401--1408},
  year={2011},
  publisher={Blackwell Publishing Ltd Oxford, UK}
}


@article{iii20083d,
  title={3D GENUS TOPOLOGY OF LUMINOUS RED GALAXIES},
  author={Got III, J Richard and Choi, Yun-Young and Park, Changbom and Kim, Juhan},
  journal={arXiv preprint arXiv:0812.1406},
  year={2008},
  publisher={Citeseer}
}

@article{Schmalzing:1997aj,
    author = "Schmalzing, Jens and Buchert, Thomas",
    title = "{Beyond genus statistics: A Unifying approach to the morphology of cosmic structure}",
    eprint = "astro-ph/9702130",
    archivePrefix = "arXiv",
    doi = "10.1086/310680",
    journal = "Astrophys. J. Lett.",
    volume = "482",
    pages = "L1--L4",
    year = "1997"
}

@article{hamilton1986topology,
  title={The topology of the large-scale structure of the universe},
  author={Hamilton, AJS and Gott III, J Richard and Weinberg, David},
  journal={The Astrophysical Journal},
  volume={309},
  pages={1--12},
  year={1986}
}


@article{melott1990topology,
  title={The topology of large-scale structure in the Universe},
  author={Melott, Adrian L},
  journal={Physics Reports},
  volume={193},
  number={1},
  pages={1--39},
  year={1990},
  publisher={Elsevier}
}

@article{szapudi1993higher,
  title={Higher order statistics of the galaxy distribution using generating functions},
  author={Szapudi, Istvan and Szalay, Alexander S},
  journal={The Astrophysical Journal},
  volume={408},
  pages={43--56},
  year={1993}
}

@article{balian1989scale,
  title={Scale-invariant matter distribution in the universe. I-Counts in cells},
 author={Balian, R and Schaeffer, R},
  journal={Astronomy and Astrophysics},
  volume={220},
  pages={1--29},
  year={1989}
}
\bibitem[\protect\citeauthoryear{Balian \& Schaeffer}{1989}]{1989A&A...220....1B} Balian R., Schaeffer R., 1989, A\&A, 220, 1



@article{white1979hierarchy,
  title={The hierarchy of correlation functions and its relation to other measures of galaxy clustering},
  author={White, Simon DM},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={186},
  number={2},
  pages={145--154},
  year={1979},
  publisher={The Royal Astronomical Society}
}

@article{Bernardeau:2001qr,
    author = "Bernardeau, F. and Colombi, S. and Gaztanaga, E. and Scoccimarro, R.",
    title = "{Large scale structure of the universe and cosmological perturbation theory}",
    eprint = "astro-ph/0112551",
    archivePrefix = "arXiv",
    reportNumber = "SACLAY-T01-142",
    doi = "10.1016/S0370-1573(02)00135-7",
    journal = "Phys. Rept.",
    volume = "367",
    pages = "1--248",
    year = "2002"
}

@article{Adamek:2016zes,
    author = "Adamek, Julian and Daverio, David and Durrer, Ruth and Kunz, Martin",
    title = "{gevolution: a cosmological N-body code based on General Relativity}",
    eprint = "1604.06065",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2016/07/053",
    journal = "JCAP",
    volume = "07",
    pages = "053",
    year = "2016"
}

@article{Hassani:2019lmy,
    author = "Hassani, Farbod and Adamek, Julian and Kunz, Martin and Vernizzi, Filippo",
    title = "{$k$-evolution: a relativistic N-body code for clustering dark energy}",
    eprint = "1910.01104",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2019/12/011",
    journal = "JCAP",
    volume = "12",
    pages = "011",
    year = "2019"
}

@article{Amendola:2016saw,
    author = "Amendola, Luca and others",
    title = "{Cosmology and fundamental physics with the Euclid satellite}",
    eprint = "1606.00180",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1007/s41114-017-0010-3",
    journal = "Living Rev. Rel.",
    volume = "21",
    number = "1",
    pages = "2",
    year = "2018"
}

@article{Fard:2017oex,
    author = "Fard, Mohammad Ansari and Baghram, Shant",
    title = "{Late time sky as a probe of steps and oscillations in primordial Universe}",
    eprint = "1709.05323",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2018/01/051",
    journal = "JCAP",
    volume = "01",
    pages = "051",
    year = "2018"
}

@article{akrami2020planck,
  title={Planck 2018 results-X. Constraints on inflation},
  author={Akrami, Yashar and Arroja, Frederico and Ashdown, M and Aumont, J and Baccigalupi, Carlo and Ballardini, M and Banday, Anthony J and Barreiro, RB and Bartolo, Nicola and Basak, S and others},
  journal={Astronomy \& Astrophysics},
  volume={641},
  pages={A10},
  year={2020},
  publisher={EDP sciences}
}

@article{Akrami:2018odb,
    author = "Akrami, Y. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. X. Constraints on inflation}",
    eprint = "1807.06211",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833887",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A10",
    year = "2020"
}


@article{ivanov2020cosmological,
  title={Cosmological parameters from the BOSS galaxy power spectrum},
  author={Ivanov, Mikhail M and Simonovi{\'c}, Marko and Zaldarriaga, Matias},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2020},
  number={05},
  pages={042},
  year={2020},
  publisher={IOP Publishing}
}


@article{alam2017clustering,
  title={The clustering of galaxies in the completed SDSS-III Baryon Oscillation Spectroscopic Survey: cosmological analysis of the DR12 galaxy sample},
  author={Alam, Shadab and Ata, Metin and Bailey, Stephen and Beutler, Florian and Bizyaev, Dmitry and Blazek, Jonathan A and Bolton, Adam S and Brownstein, Joel R and Burden, Angela and Chuang, Chia-Hsun and others},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={470},
  number={3},
  pages={2617--2652},
  year={2017},
  publisher={Oxford University Press}
}

@article{Alam:2016hwk,
    author = "Alam, Shadab and others",
    collaboration = "BOSS",
    title = "{The clustering of galaxies in the completed SDSS-III Baryon Oscillation Spectroscopic Survey: cosmological analysis of the DR12 galaxy sample}",
    eprint = "1607.03155",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1093/mnras/stx721",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "470",
    number = "3",
    pages = "2617--2652",
    year = "2017"
}


@article{shi2016mapping,
  title={Mapping the real-space distributions of galaxies in sdss dr7. i. two-point correlation functions},
  author={Shi, Feng and Yang, Xiaohu and Wang, Huiyuan and Zhang, Youcai and Mo, HJ and Van den Bosch, Frank C and Li, Shijie and Liu, Chengze and Lu, Yi and Tweed, Dylan and others},
  journal={The Astrophysical Journal},
  volume={833},
  number={2},
  pages={241},
  year={2016},
  publisher={IOP Publishing}
}


@article{wang2013sdss,
  title={The SDSS galaxy angular two-point correlation function},
  author={Wang, Y and Brunner, RJ and Dolence, JC},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={432},
  number={3},
  pages={1961--1979},
  year={2013},
  publisher={Oxford University Press}
}


@article{sanchez2012clustering,
  title={The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: cosmological implications of the large-scale two-point correlation function},
  author={S{\'a}nchez, Ariel G and Sc{\'o}ccola, Claudia G and Ross, AJ and Percival, W and Manera, M and Montesano, F and Mazzalay, X and Cuesta, AJ and Eisenstein, DJ and Kazin, E and others},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={425},
  number={1},
  pages={415--437},
  year={2012},
  publisher={Blackwell Science Ltd Oxford, UK}
}

@article{Sanchez:2012sg,
    author = "Sanchez, Ariel G. and others",
    title = "{The clustering of galaxies in the SDSS-III Baryon Oscillation Spectroscopic Survey: cosmological implications of the large-scale two-point correlation function}",
    eprint = "1203.6616",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1111/j.1365-2966.2012.21502.x",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "425",
    pages = "415",
    year = "2012"
}


@article{aghanim2020planck,
  title={Planck 2018 results-VI. Cosmological parameters},
  author={Aghanim, Nabila and Akrami, Yashar and Ashdown, M and Aumont, J and Baccigalupi, C and Ballardini, M and Banday, AJ and Barreiro, RB and Bartolo, N and Basak, S and others},
  journal={Astronomy \& Astrophysics},
  volume={641},
  pages={A6},
  year={2020},
  publisher={EDP sciences}
}

@article{Aghanim:2018eyx,
    author = "Aghanim, N. and others",
    collaboration = "Planck",
    title = "{Planck 2018 results. VI. Cosmological parameters}",
    eprint = "1807.06209",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201833910",
    journal = "Astron. Astrophys.",
    volume = "641",
    pages = "A6",
    year = "2020"
}

@article{hinshaw2013nine,
  title={Nine-year Wilkinson Microwave Anisotropy Probe (WMAP) observations: cosmological parameter results},
  author={Hinshaw, Gary and Larson, D and Komatsu, Eiichiro and Spergel, David N and Bennett, CLaa and Dunkley, Joanna and Nolta, MR and Halpern, M and Hill, RS and Odegard, N and others},
  journal={The Astrophysical Journal Supplement Series},
  volume={208},
  number={2},
  pages={19},
  year={2013},
  publisher={IOP Publishing}
}

@article{Sheth:1999mn,
  title={Large-scale bias and the peak background split},
  author={Sheth, Ravi K and Tormen, Giuseppe},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={308},
  number={1},
  pages={119--126},
  year={1999},
  publisher={The Royal Astronomical Society}
}

@article{klypin2016multidark,
  title={MultiDark simulations: the story of dark matter halo concentrations and density profiles},
  author={Klypin, Anatoly and Yepes, Gustavo and Gottl{\"o}ber, Stefan and Prada, Francisco and Hess, Steffen},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={457},
  number={4},
  pages={4340--4359},
  year={2016},
  publisher={The Royal Astronomical Society}
}

@article{riebe2013multidark,
  title={The MultiDark database: release of the Bolshoi and MultiDark cosmological simulations},
  author={Riebe, Kristina and Partl, Adrian M and Enke, Harrya and Forero-Romero, Jaimea and Gottl{\"o}ber, Stefana and Klypin, Anatolyb and Lemson, Gerardc and Prada, Franciscod and Primack, Joel R and Steinmetz, Matthiasa and others},
  journal={Astronomische Nachrichten},
  volume={334},
  number={7},
  pages={691--708},
  year={2013},
  publisher={Wiley Online Library}
}

@article{tempel2014flux,
  title={Flux-and volume-limited groups/clusters for the SDSS galaxies: catalogues and mass estimation},
  author={Tempel, E and Tamm, A and Gramann, M and Tuvikene, T and Liivam{\"a}gi, LJ and Suhhonenko, I and Kipper, R and Einasto, M and Saar, E},
  journal={Astronomy \& Astrophysics},
  volume={566},
  pages={A1},
  year={2014},
  publisher={EDP Sciences}
}

@article{lacey1994merger,
  title={Merger rates in hierarchical models of galaxy formation--II. Comparison with N-body simulations},
  author={Lacey, Cedric and Cole, Shanu},
  journal={Monthly Notices of the Royal Astronomical Society},
  volume={271},
  number={3},
  pages={676--692},
  year={1994},
  publisher={The Royal Astronomical Society}
}

@article{schneider2020baryonic,
  title={Baryonic effects for weak lensing. Part I. Power spectrum and covariance matrix},
  author={Schneider, Aurel and Stoira, Nicola and Refregier, Alexandre and Weiss, Andreas J and Knabenhans, Mischa and Stadel, Joachim and Teyssier, Romain},
  journal={Journal of Cosmology and Astroparticle Physics},
  volume={2020},
  number={04},
  pages={019},
  year={2020},
  publisher={IOP Publishing}
}

@article{york2000sloan,
  title={The sloan digital sky survey: Technical summary},
  author={York, Donald G and Adelman, J and Anderson Jr, John E and Anderson, Scott F and Annis, James and Bahcall, Neta A and Bakken, JA and Barkhouser, Robert and Bastian, Steven and Berman, Eileen and others},
  journal={The Astronomical Journal},
  volume={120},
  number={3},
  pages={1579},
  year={2000},
  publisher={IOP Publishing}
}

@article{ahn2014tenth,
  title={The tenth data release of the sloan digital sky survey: First spectroscopic data from the sdss-iii apache point observatory galactic evolution experiment},
  author={Ahn, Christopher P and Alexandroff, Rachael and Prieto, Carlos Allende and Anders, Friedrich and Anderson, Scott F and Anderton, Timothy and Andrews, Brett H and Aubourg, {\'E}ric and Bailey, Stephen and Bastien, Fabienne A and others},
  journal={The Astrophysical Journal Supplement Series},
  volume={211},
  number={2},
  pages={17},
  year={2014},
  publisher={IOP Publishing}
}

@article{Ahn:2013gms,
    author = "Ahn, Christopher P. and others",
    collaboration = "SDSS",
    title = "{The Tenth Data Release of the Sloan Digital Sky Survey: First Spectroscopic Data from the SDSS-III Apache Point Observatory Galactic Evolution Experiment}",
    eprint = "1307.7735",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    doi = "10.1088/0067-0049/211/2/17",
    journal = "Astrophys. J. Suppl.",
    volume = "211",
    pages = "17",
    year = "2014"
}

@article{Rahvar:2013xya,
    author = "Rahvar, Sohrab and Baghram, Shant and Afshordi, Niayesh",
    title = "{Transient Weak-Lensing by Cosmological Dark Matter Microhaloes}",
    eprint = "1310.5412",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.89.063001",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "6",
    pages = "063001",
    year = "2014"
}

@article{Baghram:2011is,
    author = "Baghram, Shant and Afshordi, Niayesh and Zurek, Kathryn M.",
    title = "{Prospects for Detecting Dark Matter Halo Substructure with Pulsar Timing}",
    eprint = "1101.5487",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "MCTP-11-05",
    doi = "10.1103/PhysRevD.84.043511",
    journal = "Phys. Rev. D",
    volume = "84",
    pages = "043511",
    year = "2011"
}

@article{Feldmann:2013hqa,
    author = "Feldmann, Robert and Spolyar, Douglas",
    title = "{Detecting Dark Matter Substructures around the Milky Way with Gaia}",
    eprint = "1310.2243",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.GA",
    doi = "10.1093/mnras/stu2147",
    journal = "Mon. Not. Roy. Astron. Soc.",
    volume = "446",
    pages = "1000--1012",
    year = "2015"
}

@article{deMartino:2020gfi,
    author = "de Martino, Ivan and Chakrabarty, Sankha S. and Cesare, Valentina and Gallo, Arianna and Ostorero, Luisa and Diaferio, Antonaldo",
    title = "{Dark matters on the scale of galaxies}",
    eprint = "2007.15539",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.3390/universe6080107",
    journal = "Universe",
    volume = "6",
    number = "8",
    pages = "107",
    year = "2020"
}

@article{Agustsson:2015iuo,
    author = "Agustsson, Ingolfur and Brainerd, Tereasa G.",
    title = "{The Spatial Distribution of Satellite Galaxies Selected from Redshift Space}",
    eprint = "1512.08521",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.GA",
    doi = "10.3847/1538-4357/aace5c",
    journal = "Astrophys. J.",
    volume = "862",
    number = "2",
    pages = "169",
    year = "2018"
}

@article{Li:2012qha,
    author = "Li, Fangda and Erickcek, Adrienne L. and Law, Nicholas M.",
    title = "{A new probe of the small-scale primordial power spectrum: astrometric microlensing by ultracompact minihalos}",
    eprint = "1202.1284",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.86.043519",
    journal = "Phys. Rev. D",
    volume = "86",
    pages = "043519",
    year = "2012"
}
